The restframe ultraviolet of superluminous supernovae -- I. Potential as cosmological probes

Superluminous supernovae (SLSNe) have been detected to $z\sim4$ and can be detected to $z\gtrsim15$ using current and upcoming facilities. SLSNe are extremely UV luminous, and hence objects at $z\gtrsim7$ are detected exclusively via their rest-frame UV using optical and infrared facilities. SLSNe have great utility in multiple areas of stellar and galactic evolution. Here, we explore the potential use of SLSNe type-I as high-redshift cosmological distance indicators in their rest-frame UV. Using a SLSNe-I sample in the redshift range $1\lesssim z\lesssim 3$, we investigate correlations between the peak absolute magnitude in a synthetic UV filter centered at 250 nm and rise time, colour and decline rate of SLSNe-I light curves. We observe a linear correlation between $M_0(250)$ and the rise time with an intrinsic scatter of 0.29. Interestingly, this correlation is further tightened ($\sigma_{int} \approx 0.2$) by eliminating those SLSNe which show a pre-peak bump in their light curve. This result hints at the possibility that the "bumpy" SLSNe could belong to a different population. Weak correlations are observed between the peak luminosity and colour indices. No relationship is found between UV peak magnitude and the decline rate in contrast to what is typically found in optical band. The correlations found here are promising, and give encouraging insights for the use of SLSNe as cosmological probes at high redshifts using standardising relations in the UV. We also highlight the importance of early, and consistent, photometric data for constraining the light curve properties.

==> tables/slsnUV_table1.tex <==
% slsnUV_table1.tex created at UT 2021-02-24 14:22:13
\begingroup
\setlength{\tabcolsep}{8pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.2} % Default value: 1
\begin{tabular}{c c c c c c c}
\hline\hline
ID & $z$ & Rest frame $\lambda$ & Filters used for & SLSN-UV test & Bumpy & Reference \\
 &  & coverage (\angstrom) & 250, 310 nm & sample &  & \\
\hline
DES15E2mlf     &    1.860 & $  1687 \rightarrow  3227 $ & \emph{r} $\rightarrow$ 250, \emph{i} $\rightarrow$ 310 & Yes     & may-be bumpy &\cite{angus2019} \\
DES14S2qri      &    1.500 & $  1930 \rightarrow  3691 $ & \emph{r} $\rightarrow$ 250, \emph{i} $\rightarrow$ 310 & Yes     & No  &\cite{angus2019} \\
DES14C1fi       &    1.302 & $  2096 \rightarrow  4009 $ & \emph{r} $\rightarrow$ 250, \emph{i} $\rightarrow$ 310 & No  & No & \cite{angus2019} \\
DES15X1noe      &    1.188 & $  2205 \rightarrow  4218 $ & \emph{r} $\rightarrow$ 250, \emph{i} $\rightarrow$ 310 & No  & may-be bumpy &\cite{angus2019} \\
DES17X1amf      &    0.920 & $  2513 \rightarrow  4807 $ & \emph{g} $\rightarrow$ 250, \emph{r} $\rightarrow$ 310 & Yes     & Bumpy & \cite{angus2019} \\
DES14X2byo      &    0.868 & $  2583 \rightarrow  4940 $ & \emph{g} $\rightarrow$ 250, \emph{r} $\rightarrow$ 310 & Yes     & No & \cite{angus2019} \\
DES16C3ggu      &    0.949 & $  2475 \rightarrow  4735 $ & \emph{g} $\rightarrow$ 250, \emph{r} $\rightarrow$ 310 & Yes  & No & \cite{angus2019} \\
DES15X3hm       &    0.860 & $  2594 \rightarrow  4962 $ & \emph{g} $\rightarrow$ 250, \emph{r} $\rightarrow$ 310 & No  & No &\cite{angus2019} \\
PS1-10awh       &    0.908 & $  2558 \rightarrow  4560 $ & \emph{g} $\rightarrow$ 250, \emph{r} $\rightarrow$ 310 & Yes     & may-be bumpy & \cite{chomiuk2011} \\
PS1-13or        &    1.520 & $  1937 \rightarrow  3452 $ & \emph{r} $\rightarrow$ 250, \emph{i} $\rightarrow$ 310 & No  & No & \cite{lunnan2018} \\
PS1-10pm        &    1.206 & $  2212 \rightarrow  3944 $ & \emph{r} $\rightarrow$ 250, \emph{i} $\rightarrow$ 310 & Yes     & Bumpy & \cite{mccrum2015} \\
PS1-11afv       &    1.407 & $  2028 \rightarrow  3615 $ & \emph{r} $\rightarrow$ 250, \emph{i} $\rightarrow$ 310 & No  & No & \cite{lunnan2018} \\
PS1-10ahf       &    1.100 & $  2950 \rightarrow  4143 $ & \emph{r} $\rightarrow$ 250, \emph{i} $\rightarrow$ 310 & No  & may-be bumpy & \cite{mccrum2015} \\
PS1-11aib       &    0.997 & $  2444 \rightarrow  4357 $ & \emph{g} $\rightarrow$ 250, \emph{r} $\rightarrow$ 310 & No  & No & \cite{lunnan2018} \\
HSC17auzg       &    1.965 & $  1610 \rightarrow  3007 $ & \emph{i} $\rightarrow$ 250, \emph{z} $\rightarrow$ 310 & Yes     & No & \cite{moriya2019} \\
HSC16adga       &    2.399 & $  1404 \rightarrow  2623 $ & \emph{i} $\rightarrow$ 250, \emph{z} $\rightarrow$ 310 & Yes     & No & \cite{moriya2019} \\
HSC16apuo       &    3.220 & $  1131 \rightarrow  2112 $ & \emph{z} $\rightarrow$ 250, & Yes     & No & \cite{moriya2019} \\
SNLS06D4eu      &    1.588 & $  1879 \rightarrow  3335 $ & \emph{r} $\rightarrow$ 250, \emph{i} $\rightarrow$ 310 & Yes     & Bumpy & \cite{howell2013} \\
SNLS07D2bv      &    1.500 & $  1945 \rightarrow  3452 $ & \emph{r} $\rightarrow$ 250, \emph{i} $\rightarrow$ 310 & Yes     & may-be bumpy & \cite{howell2013} \\
SN2213-1745     &    2.046 & $  1596 \rightarrow  2529 $ & \emph{i} $\rightarrow$ 250, & No  & No & \cite{Cooke2012} \\
%SN1000+0216     &    3.899 & $   992 \rightarrow  1572 $ & \emph{i} $\rightarrow$ 250, & No  & \cite{Cooke2012} \\
SN2017egm       &    0.030 & $  1871 \rightarrow  4264 $ & \emph{uvw1} $\rightarrow$ 250, \emph{U} $\rightarrow$ 310 & Yes     & may-be bumpy & \cite{nicoll2017} \\
SN2015bn        &    0.114 & $  1730 \rightarrow  3942 $ & \emph{uvw1} $\rightarrow$ 250, \emph{U} $\rightarrow$ 310 & No  & Bumpy & \cite{nicoll_2015bn} \\
\hline
\end{tabular}
\endgroup
